GRAFENNE: Learning on Graphs with Heterogeneous and Dynamic Feature Sets

Graph neural networks (GNNs), in general, are built on the assumption of a static set of features characterizing each node in a graph. This assumption is often violated in practice. Existing methods partly address this issue through feature imputation. However, these techniques (i) assume uniformity of feature set across nodes, (ii) are transductive by nature, and (iii) fail to work when features are added or removed over time. In this work, we address these limitations through a novel GNN framework called GRAFENNE. GRAFENNE performs a novel allotropic transformation on the original graph, wherein the nodes and features are decoupled through a bipartite encoding. Through a carefully chosen message passing framework on the allotropic transformation, we make the model parameter size independent of the number of features and thereby inductive to both unseen nodes and features. We prove that GRAFENNE is at least as expressive as any of the existing message-passing GNNs in terms of Weisfeiler-Leman tests, and therefore, the additional inductivity to unseen features does not come at the cost of expressivity. In addition, as demonstrated over four real-world graphs, GRAFENNE empowers the underlying GNN with high empirical efficacy and the ability to learn in continual fashion over streaming feature sets.

==> 02_related.tex <==
% \section{Related Work}


% \subsection{Graph Neural Networks with Missing features}
%  One line of work utilized matrix completion to to reconstruct the feature matrix which is then used for downstream task. Optimization and learning based  approaches \cite{hu2008collaborative,koren2009matrix} have been proposed to solve the matrix completion problem. However, they do not consider the underlying graph structure. Graph matrix completion extends the above approaches to make use of an underlying graph. Most of these approaches are computationally intensive and do not scale well beyond graph with 1K nodes. Moreover, the aim of these approaches is to reconstruct the missing features of the matrix instead our focus is directly learning a GNN with missing node features. More recently, feature propagation was used\cite{rossi2021unreasonable} to performing  diffusion-based feature reconstruction step and then reconstructued feature matrix was used to train GNN for downstream tasks. 

% Among techniques which learn on GNNs with missing node features, the recently proposed GCNMF\cite{taguchi2021graph} adapts to handle missing node features by representing  missing data with a Gaussian mixture model.
% PaGNN\cite{jiang2020incomplete} is a GNN-based model which uses  message-passing scheme to propagate only the observed features between nodes. While these approaches show reasonable performance on low feature missing rates, however they do not fare well when the percentage of missing features is high\cite{rossi2021unreasonable}. 

% \subsection{Continual learning}
% The goal of continual learning is to learn to adapt to new data in a streaming scenario while consolidating the knowledge learned from previous data to prevent catastrophic forgetting. Many techniques have been proposed to handle this scenario. The first one's being replay-based where a subset of old data samples are replayed from a memory buffer while learning a new task
% %\cite{ICARL,GEM}. 
% Second is regularization based technique which learns importance of weights of neural model for each task and prevent significant changes on them. Recently, some progress has been made to intelligently expand the neural network when the current capacity of the model is not sufficient to learn new tasks without causing forgetting of earlier one's. \textcolor{red}{conclude this para}


% \subsection{Continual Learning for GNNs}
% \textcolor{red}{add what task is solved in each }

% Recently there has been interest in developing GNNs in the continual settings. \cite{zhou2020continual} applied experience-replay of past samples while learning on new data. \cite{liu2021overcoming} utilized a memory-aware synapse framework(MAS) to learn  importance of each model parameter for each task. The method penalizes changes to these parameters while learning new tasks to prevent forgetting. \cite{wang2020streaming} developed a mixture of data replaying and Elastic Weight Consolidation(EWC) to continually learn on streaming graphs. While these techniques have shown good performance on the task in hand such as node classification et., however, these studies  were limited to either structural updates or incremental class-learning scenario.

